Positional Encoding Augmented GAN for the Assessment of Wind Flow for Pedestrian Comfort in Urban Areas

Approximating wind flows using computational fluid dynamics (CFD) methods can be time-consuming. Creating a tool for interactively designing prototypes while observing the wind flow change requires simpler models to simulate faster. Instead of running numerical approximations resulting in detailed calculations, data-driven methods and deep learning might be able to give similar results in a fraction of the time. This work rephrases the problem from computing 3D flow fields using CFD to a 2D image-to-image translation-based problem on the building footprints to predict the flow field at pedestrian height level. We investigate the use of generative adversarial networks (GAN), such as Pix2Pix [1] and CycleGAN [2] representing state-of-the-art for image-to-image translation task in various domains as well as U-Net autoencoder [3]. The models can learn the underlying distribution of a dataset in a data-driven manner, which we argue can help the model learn the underlying Reynolds-averaged Navier-Stokes (RANS) equations from CFD. We experiment on novel simulated datasets on various three-dimensional bluff-shaped buildings with and without height information. Moreover, we present an extensive qualitative and quantitative evaluation of the generated images for a selection of models and compare their performance with the simulations delivered by CFD. We then show that adding positional data to the input can produce more accurate results by proposing a general framework for injecting such information on the different architectures. Furthermore, we show that the models performances improve by applying attention mechanisms and spectral normalization to facilitate stable training.

==> chapters/00-abstract/01-additional-abstract.tex <==
% Graphical abstract
\begin{graphicalabstract}
\includegraphics[width=1.0\textwidth]{figs/Methods/training-procedure.png}
\end{graphicalabstract}

% Hightlights
\begin{highlights}
\item Using state-of-the art GAN architectures for image-to-image translation to learn the underlying RANS equations from fluid dynamics.
\item Injecting positional information into the architectures improves results
\item ...??
\end{highlights}


==> chapters/03-methods/01-objective.tex <==
\subsection{Objective}

As stated above, we optimize our model using two losses; adversarial- and supervised losses. The adversarial loss can be expressed as, similar to as in cGAN without the random noise vector:


\begin{equation}
\mathcal{L}_{adv}(G,D) =  \mathbb{E}_{x, y}[\log D(x, y)] + \mathbb{E}_{x}[\log (1-D(x, G(x)))].
\label{eq:L_adv}
\end{equation}

We want our predictions to be deterministic concerning the geometry and do therefore not include any random noise. The supervised loss, using L1-distance, can be formalized as 

\begin{equation}
\mathcal{L}_{L1}(G) = \mathbb{E}_{x, y} || G(x) - y ||_1.
\end{equation}

Together with \autoref{eq:L_adv}, this loss will push our generator to generate outputs similar to the real simulations. Its objective is now not only to fool the discriminator but to generate images close to the ground truth \cite{pathak2016context}. We get our final objective,

\begin{equation}
    G^* = \arg \min_G \max_D \mathcal{L}_{adv}(G,D) + \lambda\mathcal{L}_{L1}(G),
\label{eq:L_final}
\end{equation}
where $\lambda$ is the constant weight for the L1 penalty term.

